A WLAV-based Robust Hybrid State Estimation using Circuit-theoretic Approach

For reliable and secure power grid operation, AC state-estimation (ACSE) must provide certain guarantees of convergence while being resilient against bad-data. This paper develops a circuit-theoretic weighted least absolute value (WLAV) based hybrid ACSE that satisfies these needs to overcome some of the limitations of existing ACSE methods. Hybrid refers to the inclusion of RTU and PMU measurement data, and the use of the LAV objective function enables automatic rejection of bad data while providing clear identification of suspicious measurements from the sparse residual vector. Taking advantage of linear construction of the measurement models in circuit-theoretic approach, the proposed hybrid SE is formulated as a LP problem with guaranteed convergence. To address efficiency, we further develop problem-specific heuristics for fast convergence. To validate the efficacy of the proposed approach, we run ACSE on large cases and compare the results against WLS-based algorithms. We further demonstrate the advantages of our solution methodology over standard commercial LP solvers through comparison of runtime and convergence performance.

==> 010introduction.tex <==
Today's central grid operators run AC state estimation (ACSE) every 5 to 15 minutes to gain situational awareness of the grid states. It takes the network topology and grid measurements as inputs and outputs grid states that include complex bus voltages and angles. Furthermore, the output of this analysis serves as the input to other critical grid analyses such as optimal power flow (OPF) and contingency analysis. Therefore, for secure and reliable grid operation and control, robust ACSE is very critical. 

Yet in practice, ACSE suffers from convergence challenges and high-residuals \cite{ercot}. Many recent works have provided insight into improving ACSE convergence and estimation quality. Some have included more grid physics into the formulation as additional network constraints \cite{hachtel}. But these suffer from convergence issues due to the nonlinearity of constraints. Others have provided algorithms that are provably convergent \cite{convexSE-PMU-zhao},\cite{convexSE-PMU-chak}; albeit almost all of them are based on grid with only phasor measurement units (PMUs); an unrealistic scenario for grids today. There also have been proposed methods for convex relaxation of the hybrid ACSE problem. For instance, \cite{convexSE-SDP-weng} convexifies the problem by reformulating the voltage magnitude $|V|$, phase angle $\delta$, and product of $V$ and $I$, in semidefinite programming (SDP) form, through matrix transformation. This method however does not scale to large scale networks. More recently to overcome the convergence and high residual limitations, researchers in \cite{SUGAR-SE-Li},\cite{SUGAR-SE-Alex} proposed a circuit theoretic ACSE approach that reduces the problem to an equality constrained quadratic programming (QP) problem by creating linear measurement models following a ‘sensitivity’ based mapping of conventional grid measurements. The approach provides a convex formulation for ACSE problem that is scalable to large networks. %However, the method is not implicitly resilient against bad-data.

%Today's power industry has also seen applications of convex SE such as ISO-NE's hybrid state estimation\cite{convexSE-ISONE}. 

%there is a circuit-theoretic approach [Li et al, Alexander] that overcomes some problems with existing commercial ACSE by formulating ACSE as a convex optimization problem while including additional physics of the grid as constraints. However, this approach lacks the ability to perform implicit bad-data detection.

%To improve convergence of the later approach with RTUs included, some recent methods have proposed convex relaxation of WLAV-based optimization problem: \reminder{our previous work} reduces the problem to a equality constrained QP by creating linear measurement models through a ‘sensitivity’ based mapping of input measurements.  \reminder{xxx} convexifies the problem by reformulating the $|V|$, phase angle, as well as product of V and I, in semidefinite programming (SDP) form, through matrix transformation. Today's power industry has also seen applications of convex SE. Examples include \reminder{New England hybrid SE, ISO in Massachusetts - This approach is non-convex.}  

Meanwhile, the quality of input measurement data and the ability of the ACSE to detect any measurement anomalies is becoming increasingly critical. Unlike traditional grid settings, where measurement noise was mostly uncorrelated white noise due to faulty meters, new vectors of coordinated measurement errors from malicious cyber-attacks are expected in future. Existing bad-data detectors (BDDs) for ACSE formulations can detect traditional bad-data but are unlikely to detect faulty measurements due to coordinated attacks \cite{fdia-review}\cite{fdia-acse} and may also fail under extreme grid scenarios. Most common amongst these are the hypothesis tests that are based on post-processing of the ACSE solution residuals \cite{traditional-BDI},\cite{robustSE-reweight},\cite{robustSE-modify}. Within these algorithms, the identification of bad data is followed by adjusting suspicious measurements and rerunning ACSE until residuals are satisfactory. Possible ways of adjustments include removing bad data, modifying \cite{robustSE-modify} bad data, or iterative reweighing least square method \cite{robustSE-reweight} where weights on suspicious measurements are set to lower values. Clearly, the iterative rerunning of the ACSE problem brings high computational burden and most such detectors are dependent on convergence robustness of the ACSE itself. Other robust estimators include least median of squares \cite{robustSE-median}, yet it is not widely adopted due to numerical difficulty in handling median.

Built on the assumption that bad data are typically sparse, researchers have also proposed the use of least absolute value (LAV) in the objective function \cite{LAVSE-dc-soliman}\cite{LAVSE-dc-Vidya}\cite{LAVSE-PMU-abur}\cite{LAVSE-PMU-abur2}. The LAV based methods enable automatic rejection of bad data, eliminating the need of iterative re-runs while providing clear identification of suspicious measurements from the sparse residual vector. Despite this desirable property, the non-differentiable L1-norm terms in LAV approach introduces additional complexity. At present, two approaches to  LAV-ACSE exist: i) those that solve highly non-convex power mismatch based ACSE with conventional RTU measurements \cite{LAVSE-dc-Vidya}\cite{LAVSE-dc-Singh-splitform}\cite{LAVSE-dc-Abur-splitform}; and ii) those that are formulated as a linear programming (LP) problem for ACSE \cite{LAVSE-PMU-abur}\cite{LAVSE-PMU-abur2} with the assumption that network only consist PMUs. These convex LAV-formulations based solely on PMUs take advantage of the linear nature of the sensors, however, ensuring PMU-observability of the grid is a conservative assumption. On the other hand, for most methods in both groups, the convergence challenges to general ACSE are equally applicable whenever we seek to include remote terminal units (RTUs) into an LAV approach. 
%the inclusion of remote terminal units (RTUs) into the LAV-approach generally cause complex non-convex solution space with high likelihood of convergence difficulties.

Therefore, to overcome challenges of existing LAV ACSE methods and develop a formulation that is applicable to realistic grid scenarios, this paper extends the previous work in \cite{SUGAR-SE-Li}\cite{SUGAR-SE-Alex} and develops a convex weighted least absolute value (WLAV) based hybrid SE. Taking advantage of the linear modeling framework for all types of measurements, we formulate the hybrid SE as a linear programming (LP) problem with guaranteed convergence while performing implicit bad-data detection. Also to solve the problem efficiently, this paper develops circuit-theoretic solution methodology with primal-dual interior point (PDIP) approach \cite{PDIP-L1norm} aided with necessary heuristics for fast convergence on large-scale systems. Finally, to demonstrate the efficacy of this approach, this paper runs ACSE experiments on large networks and compare solution times and performance against simplex method and other general-purpose PDIP solvers.



==> table.tex <==
\begin{table}[ht]
\centering
\caption{Magnitude of error term $|n_i|$ at each bus (CASE14)}
\begin{tabularx}{0.8\linewidth}{lll}
\toprule
{\bf Bus ID} & {\color{red} \bf WLAV-SE} &{\bf WLS-SE}\\
\midrule
1 &  0 &  0\\
\midrule
2 &   0.009  &  0.124\\
\midrule
3 &  0  &  0.115\\
\midrule
4 &  0.065 &  0.121\\
\midrule
5 &  0  &  0.131\\
\midrule
6 (bad) &  \color{red}1.095  &  0.313\\
\midrule
8 & 0.002   &  0.027\\
\midrule
9 & 0.0  &  0.090\\
\midrule
10 & 0.0  &  0.113\\
\midrule
11 & 0.0  &  0.059\\
\midrule
12 &  0.024  &  0.155\\
\midrule
13 &  0.0  &  0.199\\
\midrule
14 (bad) &  \color{red}0.658  &  0.306\\
\midrule
{\bf MSE} &  \color{red}{\bf 0.042}  & {\bf 0.090} \\
\bottomrule
\end{tabularx}
\label{table:case14}
\end{table}
